Grad-StyleSpeech: Any-speaker Adaptive Text-to-Speech Synthesis with Diffusion Models

There has been a significant progress in Text-To-Speech (TTS) synthesis technology in recent years, thanks to the advancement in neural generative modeling. However, existing methods on any-speaker adaptive TTS have achieved unsatisfactory performance, due to their suboptimal accuracy in mimicking the target speakers' styles. In this work, we present Grad-StyleSpeech, which is an any-speaker adaptive TTS framework that is based on a diffusion model that can generate highly natural speech with extremely high similarity to target speakers' voice, given a few seconds of reference speech. Grad-StyleSpeech significantly outperforms recent speaker-adaptive TTS baselines on English benchmarks. Audio samples are available at https://nardien.github.io/grad-stylespeech-demo.

==> texts/2_related_work.tex <==
\section{Related Work}
We summarize previous works on any-speaker adaptive TTS in this section.

\textbf{Few-shot Approach}
Sample-Efficient Adaptation~\cite{SEA} and AdaSpeech~\cite{AdaSpeech} are primal works which suggest the fine-tuning of the representative speaker vector for the unseen speaker adaptation.
Moreover, AdaSpeech~\cite{AdaSpeech} introduces the speaker-conditional layer normalization to efficiently fine-tune the transformer-based architecture.

\textbf{Zero-shot Approach}
Previous works~\cite{NeuralVoiceCloning, StyleSpeech, YourTTS} leverage the speaker encoder that maps the reference speech of the target speaker into the fixed-size vector, instead of using the pre-defined set of speaker vectors. 
This property enables them to generalize to unseen speaker only with the single reference speech and without any parameter update.
Meta-StyleSpeech~\cite{StyleSpeech} utilizes the Style-Adaptive Layer Normalization (SALN) for style-adaptive synthesis and utilizes the meta-learning for better generalization on the unseen speakers.
Recently, YourTTS~\cite{YourTTS} introduce the any-speaker adaptive TTS which show the remarkable zero-shot adaptation performance.
Unlike to previous works, we focus to develop the any-speaker adaptive TTS system based on the score-based diffusion models~\cite{SDE} which have shown the decent performance on the image generation tasks.
